Query-Driven Sampling for Collective Entity Resolution

Probabilistic databases play a preeminent role in the processing and management of uncertain data. Recently, many database research efforts have integrated probabilistic models into databases to support tasks such as information extraction and labeling. Many of these efforts are based on batch oriented inference which inhibits a realtime workflow. One important task is entity resolution (ER). ER is the process of determining records (mentions) in a database that correspond to the same real-world entity. Traditional pairwise ER methods can lead to inconsistencies and low accuracy due to localized decisions. Leading ER systems solve this problem by collectively resolving all records using a probabilistic graphical model and Markov chain Monte Carlo (MCMC) inference. However, for large datasets this is an extremely expensive process. One key observation is that, such exhaustive ER process incurs a huge up-front cost, which is wasteful in practice because most users are interested in only a small subset of entities. In this paper, we advocate pay-as-you-go entity resolution by developing a number of query-driven collective ER techniques. We introduce two classes of SQL queries that involve ER operators --- selection-driven ER and join-driven ER. We implement novel variations of the MCMC Metropolis Hastings algorithm to generate biased samples and selectivity-based scheduling algorithms to support the two classes of ER queries. Finally, we show that query-driven ER algorithms can converge and return results within minutes over a database populated with the extraction from a newswire dataset containing 71 million mentions.

==> content/revisionreviews.tex <==

\onecolumn




\section{Reviewer Comments}

We would like to thank all three reviewers for their insightful and perceptive reviews.
In this section, we address comments by reviewers and point to places in the paper where these
comments are addressed.



\subsection{Summary of Changes}




\subsection{Assigned Reviewer 1}

\subsubsection{Summary}
\thereviewer{%
This chapter outlines an approach to query-driven entity resolution with two contributions:
a taxonomy of how the query-driven entity resolution can be driven by simple queries
(e.g., selections or simple joins). This is important as it identifies important special use
cases for these types of systems. It then motivates some specific optimizations for these queries
in MCMC applications.}


\thereviewer{%
The technical treatment in the paper is not as systematic as it could be.
Since query-driven ER has been described before, the first natural question is the tension between
query driven and non-query driven. 
Where does one draw the line?
What are the factors?
}

\subsubsection{Strong Points}


\thereviewer{%
Interesting problem with a very nice tie in from the application to the end engineering.
}

\thereviewer{%
The paper defines a taxonomy for how to think about a class of these entity resolution problems.
}


\subsubsection{Weak Points}


\thereviewer{%
The novelty of the optimizations and their evaluation against other state of the art methods is 
somewhat superficial. There are other joint inference approaches that have been published in 
related conferences (with implementations), but this chapter does not compare to any of them---even 
in the related work. Perhaps these optimizations interfere with other types of optimizations in 
the literature? Chromatic samplers? 
}

This is a good point and a common area for confusion.
Here we explain our choice to limit our experiments to Metropolis Hastings variation of the
standard MCMC algorithm.

This chapter  defines an optimization approach for the collective entity resolution model.
The ER model is a highly correlated pairwise model that we represent as factor graph.
The computation needed to perform Gibbs in this model is prohibitively expensive. 

Several sampling optimization in the KDD/SIGMOD family of conferences, 
such as the chromatic sampler \cite{gonzalez2011parallel, Chechetka+Guestrin:aistats10qsbp}
optimize the Gibbs sampler. 
The Gibbs method, a special case of MCMC Metropolis Hastings, have been known to perform poorly in
highly dependent structures \cite{qam}.
More specifically, when using Gibbs one needs to compute the full conditional probability of the model.
This is extremely expensive to compute over the ER model \cite{qam}.
The MCMC-MH has an acceptance score that is a ratio that removes the need to compute
this normalization constant ($Z$).
We emphasized this point in Section~\ref{sec:inferencefactorgraphs}.

Other non-Gibbs specific optimizations such as Type-based MCMC \cite{Liang:2010:TM:1857999.1858081} are
complementary to our proposed methods.
%These methods are dependent on rich feature sets.
While we discuss them in the related work section we do not perform experiments against them
because they are too feature dependent and experiments would not be fair comparisons.


%Additionally, we look to to focus the sampling over query nodes.
%In our scenario a query node is an example mention. 
%Defining what constitutes a query node in 
%This sampling optimization is good in general but defining what a query nodes 
%in this model is complex and deserves its own paper. 


\thereviewer{%
The paper does an incomplete job of related work. There is much more related work about both how 
sampling using database techniques like materialization and page layout. Frankly, the related 
work is skewed toward one of the groups working in this area leaving out many others. I think the 
work mentioned in the text is interesting, but it does not cover the range of approaches to this 
problem. For example, even vanilla MCMC algorithms can vary in their wall clock performance 
tremendously and this has been studied in the database and KDD communities.
}

This is a valid concerned expressed by the reviewers.

This chapter is broad and covers several works with different optimizations.
The entity resolution problem was identified as an exciting and relevant problem in the database
community \cite{ervldb12tutorial}.
We were forced by page limit constraints to summarize years of contributions;
We pointed readers to the most recent tutorial on the subject that (we believe) does 
that best job of giving a longitude description of work in entity resolution \cite{ervldb12tutorial}. 

%We did not focus on the implementation techniques involved in specific sampling because
%we wanted to isolate the performance benefits of the sampling customizations from the 
%engineering optimizations.

Another related area of work the database community is fond of is in-database sampling
and materialization.
Our comparison to this work was noted by the review and we added it to the related work section.
We compare our this chapter with two previous papers \cite{Zhang:2013:THG:2463676.2463702, Cai:2013:SDM:2463676.2465283}.

% TODO compare our work with chris jermaine's and chris re's

%{\added {Chris Jermaine SimSQL/MCDB, Chris Re: Towards High-Throughput Gibbs Sampling at Scale:
%A Study across Storage Managers }}
%\cite{Zhang:2013:THG:2463676.2463702, Cai:2013:SDM:2463676.2465283}. 

% ADD This...

Zhang and Re \cite{Zhang:2013:THG:2463676.2463702} discuss database methods and optimizations for
Gibbs sampling over factor graphs at scale.
Cai et al. \cite{Cai:2013:SDM:2463676.2465283}  describes a system that allows for efficient
simulation using a Gibbs sampler.
Our work provides algorithmic improvements for large-scale sampling using metropolis hastings.
We added a discussion of problems encountered when performing query-driven ER at scale.
The two previous paper explore Gibbs sampling as the foundational sampling method and this method
has been proven not to work well for our pairwise ER model.

A similar paper by Wick et al. \cite{Wick:2010:SPD:1920841.1920942} discuss an appropriate method
for Metropolis Hastings sampling in the database.

We compare our techniques to this chapter in section \ref{}.


\subsubsection{Justification of Recommendation}


\thereviewer{%
The paper does demonstrate that there are interesting techniques that one can do with the 
samplers for these specific operations (which are well motivated).
 The paper has interesting ideas, but it is explored in a somewhat unsatisfying way.
}

\thereviewer{%
Also the concept of query-driven entity resolution is a classic one
that has occurred again recently. Some citations are here:
}


\textit{%
\begin{itemize}
\item Altwaijr et al. Query-driven approach to entity resolution. VLDB13.
\item Grant et al. MADden: Query-Driven Statistical Text Analytics, CIKM12.
\end{itemize}
}

Thanks for this comment, you are correct in saying the `query-driven' concept is not 
in itself new. Further, you are correct that the idea of query-driven entity resolution
has been published in related venues.
However, in the two aforementioned papers and this current one, the actualization 
of query-driven is different.

In Grant et al.\ query-driven is being able to execute statistical text analytics tasks
using a declarative query interface such as SQL. 

In Altwaijr et al.\ the authors allow define predicates in an sql query while our techniques
use an example mention as the query.
The difference in these two approaches are the same as implementing a knn for a query (Our paper)
and specifing predicates for selection (Altwaijr et al.)
Our techniques were develop before the publishing of this chapter and the technique are complimentary
but orthogonal.

This confusion is present because we do not clearly define a query.
We added a more explicit definition in section \ref{}.






\thereviewer{%
The underlying sophistication and amount of preprocessing done on
the ER model seems to be a major factor that is somewhat
incompletely described. 
}

The cost of building an index for each query mention is constant with respect to the
number of mentions in the corpus. We hint at this fact in Section \ref{}(5.4)
Due to space considerations we did not discuss this fact further in the paper.

The other preprocessing tasks such as building indexes are performed offline 
and used for each of the four algorithms. Because this preprocessing code is 
performed once for many runs we do node we discuss this time is simply amortized
except in figure \ref{}(5). 

To address these concerns we further discuss the preprocessing involved in the
data path implementation in section \ref{}



\thereviewer{%
One could materialize a huge amount of computation up front
(essentially the entire database) or one could be lazy about the
entire computation (a purely query driven approach). However, this
paper selects something in the middle. These lazy and eager styles
of materialization have been studied in databases and for samplers
for a while. It would be helpful to position this work within that
space. Moreover, this tradeoff space is not explored here. 
}

There seems to be some confusion on what pre computation is done with query-driven
techniques.
The only pre computation performed is pairwise deterministic checks scores between
query nodes and the other mentions in the data set.
Given a set of $n$ mentions in a database there are $2^n$ possible arrangements
of resolved entities.
The amount of pairwise pre computation we perform is $q \cdot n$ where $q$ is the number
of query nodes in the set.
In addition, a common optimization task is co pre-compute the pairwise distance matrix
of a set of mentions ($n \cdot n$).

In entity resolution it is not possible to pre materialize any possible states because the
possible subsets are $2^n$. This is the whole motivation for using MCMC-MH to explore the
state space, there are too many possibilities to count.

We use the pairwise scores between the query node and the mentions in the data set as
a heuristic to more quickly find a better state.

What we did not explore in the paper is the idea that every node is a query and we
can use the pairwise distance matrix to see the influence function.
We address this in the current revision by scaling the number of query nodes to
X in the new experiments in section \ref{}.

For these reasons, and the ones mentions above why we do not use gibbs sampling,
we also do not aim to materialize sample as done in elementary
\cite{Chrie Re: Towards High-Throughput Gibbs Sampling at Scale:
A Study across Storage Managers}

Many of the optimization techniques used in gibbs do not translate to the MCMC model.





\thereviewer{%
The validation is incomplete as it would be interesting to know how well this performs on defined 
tasks (e.g., any of the KBP tasks). The NY times data set is very rich and interesting, but there 
are others with more structure that could provide interesting test cases. This setup is clean but 
it does not look realistically like what people have in these settings (the schema is much too 
simple). The complexity of the schema is not evaluated. 
}

\thereviewer{%
Although the paper focuses on large data sets, the gigaword corpus is small (less than a gig). 
There are no size stats in the experiments.
}


In the new experiments described in the paper we produce a results over the largest data set
published that contains truth data.
The numbers published by the paper can be used as a baseline for many other  works.

This setup described in this chapter is common is a typical view where entity resolution
is used in the pipeline.
We simplify many details to focus on the important parts.
Without loss of generality, we use the context attribute as a catch all to describe
the many other possible fields.




\subsubsection{Concrete Revisions}
\thereviewer{%
1. Include a more complete description of related work in this area and position the 
current optimizations against the other class of algorithms (namely from both the SIGMOD and VLDB 
communities in this space) It would also help to crisply position the work within this space and 
have a stronger novelty statement. The focus of this chapter is on the optimization of the 
underlying tasks. There are other ways to optimize aside from being query driven that have been 
considered, but are not discussed in this chapter. To what extent are these subsumed or unrelated? 
}


\thereviewer{%
2. Please include additional experiments over a more structured set of data 
(e.g., http://www.nist.gov/tac/2013/KBP/) The number and variety of data sets is a bit too low to 
draw strong experimental conclusions. The data sets in this chapter allow one to look at a narrow 
entity resolution process, but often this is part of a much larger process and it's unclear if 
optimizing this part of the process helps the overall extraction or integration process. Showing 
a more complete application here may help identify this tradeoff more 
clearly.
}


\thereviewer{%
3. Please identify the cross over point from query-driven to batch mode and what are the main 
factors in this decision. I would suggest adding a paragraph in the body about where this cross 
over point occurs and then an experiment (or two) that support where this crossover point occurs 
on the different data sets. 
}

\thereviewer{%
To make room for the longer discussion and enhanced experiments, I would suggest shrinking the 
figures.
}



%--------------------------------------------------------------------------------------------------
\subsection{Assigned Reviewer 2}


\subsubsection{Summary}


\subsubsection{Strong Points}


\subsubsection{Weak Points}


\subsubsection{Justification of Recommendation}


\subsubsection{Concrete Revisions}



%--------------------------------------------------------------------------------------------------
\subsection{Assigned Reviewer 3}

\subsubsection{Summary}


\subsubsection{Strong Points}


\subsubsection{Weak Points}


\subsubsection{Justification of Recommendation}


\subsubsection{Concrete Revisions}



\twocolumn





